Structured Partial Stochasticity in Bayesian Neural Networks

Bayesian neural network posterior distributions have a great number of modes that correspond to the same network function. The abundance of such modes can make it difficult for approximate inference methods to do their job. Recent work has demonstrated the benefits of partial stochasticity for approximate inference in Bayesian neural networks; inference can be less costly and performance can sometimes be improved. I propose a structured way to select the deterministic subset of weights that removes neuron permutation symmetries, and therefore the corresponding redundant posterior modes. With a drastically simplified posterior distribution, the performance of existing approximate inference schemes is found to be greatly improved.

==> images/nodes1.tex <==
\begin{tikzpicture}[x=2.5cm,y=1.0cm]
  \readlist\Nnod{5,7,3} % number of nodes per layer
  % \Nnodlen = length of \Nnod (i.e. total number of layers)
  % \Nnod[1] = element (number of nodes) at index 1
  \foreachitem \N \in \Nnod{ % loop over layers
    % \N     = current element in this iteration (i.e. number of nodes for this layer)
    % \Ncnt  = index of current layer in this iteration
    \foreach \i [evaluate={\x=\Ncnt; \y=\N/2-\i+0.5; \prev=int(\Ncnt-1);}] in {1,...,\N}{ % loop over nodes to draw each one
      \ifnum\Ncnt=2 % check if it's the second layer
        \node[mynode] (N\Ncnt-\i) at (\x,\y) {$h_\i$}; % neuron name is h\i
      \else
        \node[mynode] (N\Ncnt-\i) at (\x,\y) {}; % no neuron name
      \fi
    }
    \foreach \i [evaluate={\x=\Ncnt; \y=\N/2-\i+0.5; \prev=int(\Ncnt-1);}] in {1,...,\N}{ % loop over nodes to draw connections 
      \ifnum\Ncnt>1 % connect to previous layer
        \foreach \j in {1,...,\Nnod[\prev]}{ % loop over nodes in previous layer
          \pgfmathsetmacro{\minwidth}{min(\N,\Nnod[\prev])}
          \ifnum\Ncnt=3
            \pgfmathsetmacro{\q}{int(\Nnod[\prev]-\j+1)}
            \pgfmathsetmacro{\p}{int(\N-\i+1)}
          \else
            \pgfmathsetmacro{\q}{int(\j)}
            \pgfmathsetmacro{\p}{int(\i)}
          \fi
          \ifnum\i<\minwidth
            \ifnum\j<\minwidth
              \ifnum\i=\j
                \draw[thick] (N\prev-\q) -- (N\Ncnt-\p); % connect arrows directly
              \fi
            \fi
          \fi
        }
      \fi % else: nothing to connect first layer
    }
  }
\end{tikzpicture}

==> images/nodes2.tex <==
\begin{tikzpicture}[x=2.5cm,y=1.0cm]
  \readlist\Nnod{5,7,3} % number of nodes per layer
  % \Nnodlen = length of \Nnod (i.e. total number of layers)
  % \Nnod[1] = element (number of nodes) at index 1
  \foreachitem \N \in \Nnod{ % loop over layers
    % \N     = current element in this iteration (i.e. number of nodes for this layer)
    % \Ncnt  = index of current layer in this iteration
    \foreach \i [evaluate={\x=\Ncnt; \y=\N/2-\i+0.5; \prev=int(\Ncnt-1);}] in {1,...,\N}{ % loop over nodes to draw each one
      \ifnum\Ncnt=2 % check if it's the second layer
        \node[mynode] (N\Ncnt-\i) at (\x,\y) {$h_\i$}; % neuron name is h\i
      \else
        \node[mynode] (N\Ncnt-\i) at (\x,\y) {}; % no neuron name
      \fi
    }
    \foreach \i [evaluate={\x=\Ncnt; \y=\N/2-\i+0.5; \prev=int(\Ncnt-1);}] in {1,...,\N}{ % loop over nodes to draw connections 
      \ifnum\Ncnt>1 % connect to previous layer
        \foreach \j in {1,...,\Nnod[\prev]}{ % loop over nodes in previous layer
          \pgfmathsetmacro{\minwidth}{min(\N,\Nnod[\prev])}
          \ifnum\Ncnt=3
            \pgfmathsetmacro{\q}{int(\Nnod[\prev]-\j+1)}
            \pgfmathsetmacro{\p}{int(\N-\i+1)}
          \else
            \pgfmathsetmacro{\q}{int(\j)}
            \pgfmathsetmacro{\p}{int(\i)}
          \fi
          \ifnum\i<\minwidth
            \ifnum\j<\minwidth
              \ifnum\i=\j
                \draw[thick] (N\prev-\q) -- (N\Ncnt-\p); % connect arrows directly
              \fi
            \fi
          \fi
        }
      \fi % else: nothing to connect first layer
    }
  }
\draw[thick, dashed] (N2-5) -- (N3-2);
\end{tikzpicture}

==> images/nodes3.tex <==
\begin{tikzpicture}[x=2.5cm,y=1.0cm]
  \readlist\Nnod{5,7,3} % number of nodes per layer
  % \Nnodlen = length of \Nnod (i.e. total number of layers)
  % \Nnod[1] = element (number of nodes) at index 1
  \foreachitem \N \in \Nnod{ % loop over layers
    % \N     = current element in this iteration (i.e. number of nodes for this layer)
    % \Ncnt  = index of current layer in this iteration
    \foreach \i [evaluate={\x=\Ncnt; \y=\N/2-\i+0.5; \prev=int(\Ncnt-1);}] in {1,...,\N}{ % loop over nodes to draw each one
      \ifnum\Ncnt=2 % check if it's the second layer
        \node[mynode] (N\Ncnt-\i) at (\x,\y) {$h_\i$}; % neuron name is h\i
      \else
        \node[mynode] (N\Ncnt-\i) at (\x,\y) {}; % no neuron name
      \fi
    }
    \foreach \i [evaluate={\x=\Ncnt; \y=\N/2-\i+0.5; \prev=int(\Ncnt-1);}] in {1,...,\N}{ % loop over nodes to draw connections 
      \ifnum\Ncnt>1 % connect to previous layer
        \foreach \j in {1,...,\Nnod[\prev]}{ % loop over nodes in previous layer
          \pgfmathsetmacro{\minwidth}{min(\N,\Nnod[\prev])}
          \ifnum\Ncnt=3
            \pgfmathsetmacro{\q}{int(\Nnod[\prev]-\j+1)}
            \pgfmathsetmacro{\p}{int(\N-\i+1)}
          \else
            \pgfmathsetmacro{\q}{int(\j)}
            \pgfmathsetmacro{\p}{int(\i)}
          \fi
          \ifnum\i<\minwidth
            \ifnum\j<\minwidth
              \ifnum\i>\j
              \else % this and above line achieves \ifnum \i <= \j
                \draw[thick] (N\prev-\q) -- (N\Ncnt-\p); % connect arrows directly
              \fi
            \fi
          \fi
        }
      \fi % else: nothing to connect first layer
    }
  }
\end{tikzpicture}

==> images/nodes4.tex <==
\begin{tikzpicture}[x=2.5cm,y=1.0cm]
  \readlist\Nnod{5,7,3} % number of nodes per layer
  % \Nnodlen = length of \Nnod (i.e. total number of layers)
  % \Nnod[1] = element (number of nodes) at index 1
  \foreachitem \N \in \Nnod{ % loop over layers
    % \N     = current element in this iteration (i.e. number of nodes for this layer)
    % \Ncnt  = index of current layer in this iteration
    \foreach \i [evaluate={\x=\Ncnt; \y=\N/2-\i+0.5; \prev=int(\Ncnt-1);}] in {1,...,\N}{ % loop over nodes to draw each one
      \ifnum\Ncnt=2 % check if it's the second layer
        \node[mynode] (N\Ncnt-\i) at (\x,\y) {$h_\i$}; % neuron name is h\i
      \else
        \node[mynode] (N\Ncnt-\i) at (\x,\y) {}; % no neuron name
      \fi
    }
    \foreach \i [evaluate={\x=\Ncnt; \y=\N/2-\i+0.5; \prev=int(\Ncnt-1);}] in {1,...,\N}{ % loop over nodes to draw connections 
      \ifnum\Ncnt>1 % connect to previous layer
        \foreach \j in {1,...,\Nnod[\prev]}{ % loop over nodes in previous layer
          \pgfmathsetmacro{\minwidth}{min(\N,\Nnod[\prev])}
          \ifnum\Ncnt=3
            \pgfmathsetmacro{\q}{int(\Nnod[\prev]-\j+1)}
            \pgfmathsetmacro{\p}{int(\N-\i+1)}
          \else
            \pgfmathsetmacro{\q}{int(\j)}
            \pgfmathsetmacro{\p}{int(\i)}
          \fi
          \ifnum\i<\minwidth
            \ifnum\j<\minwidth
              \ifnum\i>\j
              \else
                \draw[thick] (N\prev-\q) -- (N\Ncnt-\p); % connect arrows directly
              \fi
            \fi
          \fi
        }
      \fi % else: nothing to connect first layer
    }
  }
\draw[thick, dashed] (N2-5) -- (N3-2);
\end{tikzpicture}

==> images/teximage.tex <==
\frame{\begin{picture}(100,100)
\put(25,50){\dashbox{.5}(10,10){$A$}}
\put(50,50){\dashbox{.5}(10,10){$B$}}
\end{picture}}

